Generating Data Augmentation samples for Semantic Segmentation of Salt Bodies in a Synthetic Seismic Image Dataset

Nowadays, subsurface salt body localization and delineation, also called semantic segmentation of salt bodies, are among the most challenging geophysicist tasks. Thus, identifying large salt bodies is notoriously tricky and is crucial for identifying hydrocarbon reservoirs and drill path planning. This work proposes a Data Augmentation method based on training two generative models to augment the number of samples in a seismic image dataset for the semantic segmentation of salt bodies. Our method uses deep learning models to generate pairs of seismic image patches and their respective salt masks for the Data Augmentation. The first model is a Variational Autoencoder and is responsible for generating patches of salt body masks. The second is a Conditional Normalizing Flow model, which receives the generated masks as inputs and generates the associated seismic image patches. We evaluate the proposed method by comparing the performance of ten distinct state-of-the-art models for semantic segmentation, trained with and without the generated augmentations, in a dataset from two synthetic seismic images. The proposed methodology yields an average improvement of 8.57% in the IoU metric across all compared models. The best result is achieved by a DeeplabV3+ model variant, which presents an IoU score of 95.17% when trained with our augmentations. Additionally, our proposal outperformed six selected data augmentation methods, and the most significant improvement in the comparison, of 9.77%, is achieved by composing our DA with augmentations from an elastic transformation. At last, we show that the proposed method is adaptable for a larger context size by achieving results comparable to the obtained on the smaller context size.

==> sections/3-Background/conditional_flow.tex <==
\subsection{Conditional Normalizing Flow Models} \label{sec:conditional-flow}

    The Conditional Normalizing Flow (CNF) is an NF extension to the conditional case.
    Thus,
        CNF extends the NF by conditioning the entire generative process on an input $y$ \cite{Ardizzone2019GuidedIG, Winkler2019LearningLW}.
    
    The goal is to estimate conditional likelihoods using conditional normalizing flows for complicated target distributions in multivariate prediction tasks.
    
    Given an input $y$ and a target $x$,
        we learn the distribution $p(x|y)$ 
        using the conditional base distribution $\pi(z_{k}|y)$ 
        and a sequence of $k$ mappings 
        $$
            % z_{k} = f_{\omega}(x,y) = f^{k}(...(f^{1}(x,y),y),y)
            z_{k} = f_{\omega}(x) = f^{k}(...(f^{1}(x)))
        $$
        % $f_{i}: X \times Y \rightarrow Z$, 
        % $f_{i}: X \rightarrow Z$, 
        which are bijective in $x$ 
        and $z_{k}$.
    Thus,
        the change of variables formula becomes:
            \begin{equation}
                \label{eq:conditional-change-of-variable-formula}
                % p(x|y) = \pi(f_{\omega}(x,y)|y)\left | det \left (\frac{\partial f_{\omega}(x,y)}{\partial x} \right ) \right |
                p(x|y) = \pi(f_{\omega}(x)|y)\left | det \left (\frac{\partial f_{\omega}(x)}{\partial x} \right ) \right |
            \end{equation}
    % The bijective mapping $f_{\omega}$ allows modelling multimodal distributions \cite{Winkler2019LearningLW}.
    
    The generative process is done by 
        first sampling $z_{k}$ from a simple base density,
        which has its parameters determined by an arbitrary function that receives $y$ as input. % (for us this is a diagonal Gaussian) 
    Then, 
        $z_{k}$ is transformed by the sequence of bijective mappings $f^{-1}_{\omega}(z_{k})$. 
        %$f^{-1}_{\omega}(z_{k}, y)$. 
    Therefore, 
        the generative process is defined as:
            \begin{equation}
                \label{eq:z-follows-p}
                % z_{k} \sim \pi(f_{\omega}(x,y)|y)
                z_{k} \sim \pi(f_{\omega}(x)|y)
            \end{equation}
            \begin{equation}
                \label{eq:x-fz}
                % x = f_{\omega}^{-1}(z_{k},y)
                x = f_{\omega}^{-1}(z_{k})
            \end{equation}

    During the training procedure,
        % $x$ and $y$ are given as inputs to the model 
        $x$ is given as inputs to the model 
        % and passed through the invertible mapping $f_{\omega}(x,y)$ 
        and passed through the invertible mapping $f_{\omega}(x)$ 
        to yield $z_{k}$.
    Then the base distribution parameters and the log-likelihood are evaluated.
    As usual, 
        in neural networks, 
        the flow and base distribution parameters are optimized using stochastic gradient descent with mini-batches. 
    
    In this work, 
        the conditional data are just binary masks,
        and since the conditioning is introduced only in the base distribution, 
        unlike in other applications, 
        in which the conditional information is also used as input 
        to (I) the affine coupling layer internal operators \cite{Ardizzone2019GuidedIG}
        and (II) to an affine projection layer \cite{Lugmayr2020SRFlowLT}.
    
    Therefore,
        the base distribution parameters are set by arbitrary functions such that:
        % we set the mean and variance as functions of $y$ such that
        \begin{equation}
            \label{eq:prior-net}
            \pi(z_{k}|y) = \mathcal{N}(z; \mu(y), \sigma(y)),
        \end{equation}
        where $\mu(y)$ and $\sigma(y)$ are the outputs of a simple convolutional neural network that uses the conditioning term $y$ as input.
        
    


==> sections/3-Background/equations/eq_change_of_variable_formula.tex <==
\begin{equation}
    \label{eq:change-of-variable-formula}
    p(x) = \pi_{Z}(f_{\omega}(x)) 
        \left | 
            det 
            \left (
                    \frac
                        { \partial f_{\omega}(x) }
                        {\partial x} 
                \right ) 
            \right |
\end{equation}

==> sections/3-Background/equations/eq_change_of_variable_formula_conditional.tex <==
\begin{equation}
    \label{eq:conditional-change-of-variable-formula}
    p(x) = \pi(f_{\omega}(x,y)|y)\left | det \left (\frac{\partial f_{\omega}(x,y)}{\partial x} \right ) \right |
\end{equation}

==> sections/3-Background/equations/eq_elbo.tex <==
\begin{equation}
    \label{eq:elbo}
    log\ p_{\theta}(x) \geq \mathbb{E}_{q} \left [\ log\ p_{\theta}(x|z)\ \right ] - \mathbb{KL}(q(z|x) || p(z)) 
\end{equation}
% In such a model, 
%     $x$ is generated by sampling from the estimated distribution $p_{\theta}(x|z)$, 
%     which is conditioned on the unobserved latent variable $z$.
%     where $\theta$ represents the neural network parameters that are learned by maximizing the lower bound defined by ELBO \ref{eq:elbo}.
    % conditioned on an unobserved latent variable $z$
    
% Moreover,
%     the posterior approximation $q_{\phi}(z|x)$ addresses the intractability of the true posterior
%     and is also done by a neural network.
    % which predicts the distribution's variational parameters.

==> sections/3-Background/equations/eq_elbo_cvae.tex <==
\begin{equation}
    \label{eq:elbo-cvae}
    log\ p_{\theta}(x|y) \geq \mathbb{E}_{q} \left [\ log\ p_{\theta}(x|z,y)\ \right ] - \mathbb{KL}(q(z|x,y) || \pi(z|y)) 
\end{equation}

==> sections/3-Background/invertible_layers/actnorm.tex <==
\subsubsection{ActNorm}
    Also introduced by the Glow model \cite{Kingma2018GlowGF},
        the ActNorm layer is proposed, 
        as an alternative to the standard batch normalization \cite{Ioffe2015BatchNA},
        for models trained with small mini-batches.
    Similar to the batch normalization, 
        the ActNorm layer performs a per-channel normalization in the network activations.
    Thus,
        the ActNorm layer performs an affine transformation to shift 
        and scale the network activations, 
        using its scale 
        and bias trainable parameters.
    
    Additionally, 
        the scale and bias parameters are initialized such that 
        the activations after the Actnorm layer have approximately zero mean 
        and unit variance.
    
    Finally, 
        the log-determinant is computed as follows:
        \begin{equation}
            \label{eq:acnorm-logdet}
            log \left | det\left ( \frac{ \partial s \odot x + b}{\partial x} \right ) \right | = w \cdot sum(log|s|)
        \end{equation}
    In equation \ref{eq:acnorm-logdet},
        $x$ is the layer input, 
        $s$ is the scale parameter, 
        $b$ is the bias parameter, 
        $\odot$ is an element-wise product operation, 
        and $w$ stands for the input width dimensions.


==> sections/3-Background/invertible_layers/coupling-layers.tex <==
\subsubsection{Affine Coupling Layers}
    
    The affine coupling layer, 
        first introduced in Nice and RealNVP \cite{Dinh2014NICENI, Dinh2016DensityEU},
        is a simple bijective layer that is simple to invert 
        and has a tractable Jacobian determinant. 
    In this layer,
        the input vector is partitioned into two halves, 
        and then one partition is updated using complex dependencies computed from the other partition.
    In the end, 
        the layer concatenates the partitions into a vector containing the same dimensions as its input. 
    Thus, 
        given $D$-dimensional input $x$ and a scalar $d < D$, 
        the affine coupling layer output $h$ follows:
            \begin{equation}
                \label{eq:affine-coupling-layer}
                h = 
                \left\{
                \begin{matrix}
                    h_{1:d} = x_{1:d}; \\ 
                    h_{d+1:D} = x_{d+1:D} \odot  exp(s(x_1:d)) + t(x_{1:d})
                \end{matrix}
                \right.
            \end{equation}
        where $s$ and $t$ 
        are functions from $\mathcal{R}^{d} \rightarrow \mathcal{R}^{D - d}$, 
        and $\odot $ is the element-wise product.
    
    The Jacobian of the transformation expressed in equation \ref{eq:affine-coupling-layer}, 
        is as follows:
            \begin{equation}
                \label{eq:affine-coupling-jacobian}
                J =  
                \begin{bmatrix}
                    \mathbb{I}_{d} & 0_{d\times(D-d)} \\ 
                    \frac{\partial h_{d+1:D}}{\partial x_{1:d}} & diag(exp(s(x_{1:d})))
                \end{bmatrix}
            \end{equation}
    In equation \ref{eq:affine-coupling-jacobian}, 
        $diag(exp(s(x_{1:d})))$ 
        is the diagonal matrix whose diagonal elements correspond to the vector 
        $s(x_{1:d}))$. 
    Since the Jacobian is upper triangular, 
        its determinant is efficiently computed as 
        $exp \left[ \sum_{j} s( x_{1:d})_{j} \right ]$.
    
    Since computing the Jacobian determinant of the affine coupling layer does not involve calculating the $s$ and $t$ Jacobians, 
        those operators are calculated by a standard neural network block that serves as the layer's backbone.
    
    Finally, 
        computing the inverse of the coupling layer is no more complex than the forward propagation, 
        and therefore, 
        sampling is as efficient as inference. 
    Equation \ref{eq:affine-coupling-layer-inverse} defines the inverse transformation of the affine coupling layer.
        \begin{equation}
            \label{eq:affine-coupling-layer-inverse}
            x = 
            \left\{
            \begin{matrix}
                x_{1:d} = h_{1:d}; \\ 
                x_{d+1:D} = (h_{d+1:D} - t(h_{1:d})) \odot  exp(-s(h_{1:d}))
            \end{matrix}
            \right.
        \end{equation}
    
    % \subsubsection*{Split and concatenation}
    % The affine coupling layer splits the input tensor $x$ into two halves, 
    %     and at the end, 
    %     the layer undoes the split by concatenating the two halves into a single tensor again.

==> sections/3-Background/invertible_layers/invertible-conv.tex <==
\subsubsection{Invertible 1 x 1 convolutions}

    The Glow model architecture \cite{Kingma2018GlowGF} proposes to replace the most commonly used fixed permutations \cite{Dinh2014NICENI, Dinh2016DensityEU} operator with a $1 \times 1$ invertible convolutional layer,
        which they claim to be a generalization of the permutation operators.
    
    In this layer,
        the convolution weight matrix is initialized as a random rotation matrix, with the same number of filters as the number of input channels $c$.
        % and the number of channels $c$ in its 
        % inputs and outputs is the same. 
        % reescrive assim ^ o que vc acha?
        
    Thus, 
        the invertible $1 \times 1$ convolution receives a tensor 
        $x \in \mathbb{R}^{w \times c}$ 
        as input and applies the convolutional operator using the weight matrix 
        $W \in \mathbb{R}^{c \times c}$ as its convolutional kernel.
    Additionally,  
        the weight matrix $W$ is initialized such that its initial log-determinant is $0$.
    
    Finally, 
        the log-determinant of this layer is computed as follows:
            \begin{equation}
                \label{eq:inv-conv-logdet}
                log \left | det\left ( \frac{\partial conv2D(h; W)}{\partial h} \right ) \right | = width \cdot log|det(W)|
            \end{equation}

        
    
    
   

==> sections/keywords.tex <==
Conditional Normalizing Flows, Variational AutoEncoders, Data Augmentation, Semantic Segmentation of Salt Bodies
